Space-filling curves of self-similar sets (II): Edge-to-trail substitution rule

It is well-known that the constructions of space-filling curves depend on certain substitution rules. For a given self-similar set, finding such rules is somehow mysterious, and it is the main concern of the present paper. Our first idea is to introduce the notion of skeleton for a self-similar set. Then, from a skeleton, we construct several graphs, define edge-to-trail substitution rules, and explore conditions ensuring the rules lead to space-filling curves. Thirdly, we summarize the classical constructions of the space-filling curves into two classes: the traveling-trail class and the positive Euler-tour class. Finally, we propose a general Euler-tour method, using which we show that if a self-similar set satisfies the open set condition and possesses a skeleton, then space-filling curves can be constructed. Especially, all connected self-similar sets of finite type fall into this class. Our study actually provides an algorithm to construct space-filling curves of self-similar sets.

==> Optimal_V1.tex <==
\bigskip

%\noindent \textbf{Appendix.} \textit{Definition of Optimal parametrization.}
%
%Let $K$ be a subset of ${\mathbb R}^d$ with Hausdorff dimension $s$, and the $s$-dimensional Hausdorff measure is positive, that is, $0<{\mathcal H}^s(K)<\infty$.
% An  onto mapping   $\psi:[0,1]\rightarrow K$ is called an
%\emph{optimal parametrization} of $K$ if the following three conditions are fulfilled.
%
%\ \ $(i)$  $\psi$ is almost one-to-one, precisely, there exist $K'\subset K$ and $I'\subset [0,1]$ such that
%  ${\mathcal H}^s(K\setminus K')={\mathcal L}([0,1]\setminus I')=0$ and $\psi:~I'\to K'$ is a bijection;
%
%  \ $(ii)$ $\psi$ is measure-preserving in the sense that
%  $$
%  {\mathcal H}^s(\psi(F))=c{\mathcal L}(F) \text{ and } {\mathcal L}(\psi^{-1}(B))=c^{-1}{\mathcal H}^s(B),
%  $$
%  for any Borel set $F\subset [0,1]$ and any Borel set $B\subset K$, where $c={\mathcal H}^s(K)$.
%
%  $(iii)$ $\psi$ is $1/s$-H\"older continuous, that is, there is a constant $c'>0$ such that
%  $$
%  |\psi(x)-\psi(y)|\leq c'|x-y|^{\frac{1}{s}} \  \text{ for all } x,y\in [0,1].
%  $$



%\begin{example}
%\textbf {The pinwheel tile.}{\rm
%This five-reptile is found  by Bandt and Mekhontsev \cite{Bandt2017}\cite{Mekhontsevwebsite}.
% The IFS is
%$$
%\begin{matrix}
%~S_1(z)=\frac{2+\mi}{5}\bar{z},\quad
%~~~S_2(z)=\frac{1-2i}{5}z+\frac{2+i}{5},\quad
%S_3(z)=\frac{-1+2i}{5}z+1,\\
%S_4(z)=\frac{2+i}{5}z+\frac{2+i}{5},
%\quad\quad S_5(z)=\frac{1-2i}{5}(-\bar{z})+\frac{4+2i}{5}.
%\end{matrix}
%$$
%
%\input{Example_Pinwheel}
%
%We choose $A=\{a_1, a_2, a_3\}=\{0, 1, 1+i\}$, the three vertice of the unit square, to be a skeleton. Let $$V=\overrightarrow{a_1a_2}+\overrightarrow{a_2a_3}+\overrightarrow{a_3a_1}=v_1+v_2+v_3$$ be the initial circle, and $V^{-1}=v_3^{-1}+v_2^{-1}+v_1^{-1}$ is the inverse circle of $V$. Let $\beta\in\{1, -1\}^5$. Then the refine graph is given by
%$$G=\cup_{i=1}^5S_i(V^{\beta_i}).$$
%To get a self-avoiding visualization, we choose $\beta=(-1,1,1,1,-1)$. (See Figure \ref{Fig_Pinwheel}(d)). According to the partition of the Eulerian path of $G$ in Figure \ref{Fig_Pinwheel}(d), we obtain the following path-substitution.
%\begin{equation}
%\left \{
%\begin{array}{l}
%v_1\mapsto S_1(v_3^{-1})+S_1(v_2^{-1})+S_2(v_1)+S_2(v_2),\\
%v_2\mapsto S_2(v_3)+S_3(v_3)+S_3(v_1)+S_5(v_3^{-1}),\\
%v_3 \mapsto S_5(v_2^{-1})+S_5(v_1^{-1})+S_4(v_2)+S_4(v_3)+S_4(v_1)+S_3(v_2)+S_1(v_1^{-1}).
%\end{array}
%\right .
%\end{equation}
%}
%
%\end{example}

